Boosting Vehicle-to-cloud Communication by Machine Learning-enabled Context Prediction

The exploitation of vehicles as mobile sensors acts as a catalyst for novel crowdsensing-based applications such as intelligent traffic control and distributed weather forecast. However, the massive increases in Machine-type Communication (MTC) highly stress the capacities of the network infrastructure. With the system-immanent limitation of resources in cellular networks and the resource competition between human cell users and MTC, more resource-efficient channel access methods are required in order to improve the coexistence of the different communicating entities. In this paper, we present a machine learning-enabled transmission scheme for client-side opportunistic data transmission. By considering the measured channel state as well as the predicted future channel behavior, delay-tolerant MTC is performed with respect to the anticipated resource-efficiency. The proposed mechanism is evaluated in comprehensive field evaluations in public Long Term Evolution (LTE) networks, where it is able to increase the mean data rate by 194% while simultaneously reducing the average power consumption by up to 54%.

==> tex/relatedWork/kpi.tex <==
% !TeX spellcheck = en_US

\section{Application Scenario and Key Performance Indicators} \label{sec:problem_definition}




\subsection{Network Quality Indicators} \label{sec:indicators}

The \LTE standard defines numerous indicators to evaluate the network quality~\cite{TS36214}.
Depending on the \UE and the operating system, only a subset is available to the application-layer.
The most common indicators are as follows:
\\
\emph{\acf{RSRP}} [\si{\dBm}] describes the average received power in resource elements, which carry the cell-specific reference signals. The value is a strong indicator for the signal strength and is internally used by the \UE to estimate the path loss.
It is independent of the cell bandwidth and any activity within the cell.
\\
\emph{\acf{RSSI}} [\si{\dBm}] describes, in contrast to \RSRP, the total received signal strength over the whole cell bandwidth. This includes the power of reference signals, control channels, payload traffic, and interference from neighboring cells.
\\	
\emph{\acf{RSRQ}} [\si{\dB}] is defined as the difference of the previous indicators:
\begin{align}
\text{RSRQ} = 10\log_{10}\left(N_\text{PRB}\right)+\text{RSRP}-\text{RSSI},\label{eq:rsrq}
\end{align}
where $N_\text{PRB}$ reflects the total cell bandwidth by means of available \PRBs.
The \RSRQ indicates the current cell load and the degree of interference by neighboring cells.
\\
%
% SINR
%
\emph{\acf{SINR}} [\si{\dB}] is defined as the difference between the signal power of received cell-specific reference signals to the background power level and the interference power in those resource elements.
\\	
\emph{\acf{CQI}} is an integer value in the range of \num{0} to \num{15}, which is computed by the \UE to inform the \eNB about the highest possible \MCS for future downlink transmissions under the current radio conditions.
The calculation of the \ac{CQI} is \emph{not specified by the standard and depends on the modem manufacturer}.
However, according to~\cite{3GPP/2016a} the reported \ac{CQI} shall guarantee a correct reception of a transport block with an error probability $\leq 0.1$.



==> tex/relatedWork/stateOfTheArt.tex <==
%\renewcommand{\arraystretch}{1.1}
\begin{table*}[h]

	\centering
	\caption{State-of-the-art approaches for vehicle detection and classification}

	%\resizebox{0.4\textwidth}{!}{%
	\begin{tabularx}{0.44\textwidth}{|X|X|}
		\hline
		
		\textbf{Approach} & \textbf{} \\ \hline
		
		Camera & ...  \\ \hline
		

	\end{tabularx}
	\label{tab:classificationApproaches}

\end{table*}


% Privacy
% Classification
% Cost
% Accuracy
% Weather
% Multi-lane
